A precision apparatus for high harmonic spectroscopy in bulk solids

High harmonic generation (HHG) in solids has emerged as a powerful spectroscopic method for resolving ultrafast electron dynamics and band structure properties across a wide range of materials. However, quantitative HHG studies require instrumentation capable of delivering stable driving fields, precise crystal alignment, and broadband detection spanning the UV to the extreme ultraviolet (EUV). Here we present an integrated apparatus engineered specifically for high-accuracy, field-strength and orientation-dependent HHG measurements in bulk solids. The system incorporates dispersion-neutral intensity-control for few-cycle pulses, a vacuum HHG module with sub-micrometer and sub-degree sample positioning, and an imaging assembly that stabilizes the focal spot position and enables spatial filtering of the emitted harmonics. A synchronized dual-spectrometer scheme provides simultaneous UV/VUV and EUV radiation detection, while absolute electric field calibration is achieved through gas-phase attosecond streaking. Together, these capabilities establish a versatile and quantitatively reliable platform for solid-state HHG spectroscopy. The methodology is broadly adaptable to various laser sources and material classes, and supports future efforts aimed at reconstructing valence-electron potentials, tracking strong-field dynamics, and mapping electronic structure with sub-cycle temporal resolution.

==> abstract.tex <==
High-harmonic generation (HHG) in solids has emerged as a powerful spectroscopic method for resolving ultrafast electron dynamics and band structure properties across a wide range of materials. However, quantitative HHG studies require instrumentation capable of delivering stable driving fields, precise crystal alignment, and broadband detection spanning the UV to the extreme ultraviolet (EUV). Here we present an integrated apparatus engineered specifically for high-accuracy, field-strength and orientation-dependent HHG measurements in bulk solids. The system incorporates dispersion-neutral intensity-control for few-cycle pulses, a vacuum HHG module with sub-micrometer and sub-degree sample positioning, and an imaging assembly that stabilizes the focal spot position and enables spatial filtering of the emitted harmonics. A synchronized dual-spectrometer scheme provides simultaneous UV/VUV and EUV radiation detection, while absolute electric field calibration is achieved through gas-phase attosecond streaking. Together, these capabilities establish a versatile and quantitatively reliable platform for solid-state HHG spectroscopy. The methodology is broadly adaptable to various laser sources and material classes, and supports future efforts aimed at reconstructing valence-electron potentials, tracking strong-field dynamics, and mapping electronic structure with sub-cycle temporal resolution.


==> detection.tex <==
\section{Detection system}
\label{sec:detection}

Comprehensive spectroscopic characterization of high harmonics requires simultaneous detection across a broad spectral range, from the UV ($\sim 3$~eV) to the EUV ($\sim 100$~eV). To achieve this, we employ a dual-spectrometer configuration consisting of a UV/VUV spectrometer and an EUV spectrometer, both operating in parallel and synchronized to the laser repetition rate.

\subsection{UV/VUV spectrometer}

The UV/VUV spectrometer (Fig.~\ref{fig:detection}a) covers the spectral range from 200 to 650~nm (1.9 to 6.2~eV) with a resolution of $\sim 0.5$~nm. It is based on a Czerny-Turner configuration with a focal length of 300~mm and a holographic grating (1200 lines/mm, blazed at 300~nm). The entrance slit width is adjustable from 10 to 200~$\mu$m, allowing a trade-off between spectral resolution and signal level.

Dispersed light is detected by a back-illuminated CCD camera (1024 $\times$ 256 pixels, pixel size 26~$\mu$m) cooled to $-40^\circ$C to minimize dark current. The camera is operated in photon-counting mode for low-signal applications or in integration mode for high-signal measurements. The quantum efficiency is $> 60\%$ across the full spectral range, and the dynamic range exceeds $10^4$ within a single exposure.

The UV/VUV spectrometer is particularly useful for detecting low-order harmonics (3rd to 9th order for 800~nm driving wavelength) and for monitoring the transmitted driving laser spectrum. It also enables measurements of harmonic polarization states by inserting a rotating polarizer before the entrance slit.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\textwidth]{media/media/image5.png}
\caption{Detection system. (a) UV/VUV spectrometer (Czerny-Turner configuration, 200--650~nm range). (b) EUV spectrometer (grazing-incidence flat-field design, 10--100~eV range). Both spectrometers operate in parallel, enabling simultaneous detection of harmonics across a broad spectral range.}
\label{fig:detection}
\end{figure}

\subsection{EUV spectrometer}

The EUV spectrometer (Fig.~\ref{fig:detection}b) covers the range from 10 to 100~eV (12 to 124~nm) with a resolution of $\sim 0.2$~eV at 50~eV. It employs a grazing-incidence flat-field design with a variable-line-spacing (VLS) grating optimized for broadband focusing\cite{Harada1980,Harada1999}. The grating (1200 lines/mm at the center, $\pm 10\%$ line-spacing variation) is coated with gold to maximize reflectivity in the EUV range.

The detector is a microchannel plate (MCP) coupled to a phosphor screen and a CCD camera. The MCP provides single-photon sensitivity and high gain ($> 10^6$), enabling detection of weak harmonic signals. The phosphor screen converts the amplified electron signal to visible light, which is imaged onto the CCD camera. The effective pixel size at the detector plane is $\sim 25~\mu$m, corresponding to a spectral resolution of $\sim 0.2$~eV.

To prevent saturation and damage of the MCP by intense low-order harmonics or scattered driving laser light, a set of thin metallic filters (Al, Zr, or combinations thereof) can be inserted before the entrance slit. These filters provide wavelength-dependent attenuation, blocking visible and UV radiation while transmitting EUV photons. The filter selection is optimized based on the expected harmonic spectrum and the sample under investigation.

\subsection{Synchronization and data acquisition}

Both spectrometers are synchronized to the laser repetition rate (typically 1--10~kHz) using a common trigger signal derived from the laser oscillator or amplifier. This ensures that harmonic spectra from individual laser shots can be recorded and analyzed separately, enabling shot-to-shot statistics and rejection of outliers caused by laser fluctuations or sample damage.

Data acquisition is controlled by a custom software interface that coordinates the spectrometer readout, stage positioning, and laser parameters. For field-strength scans, the software automatically adjusts the intensity control module (Sec.~III) and records spectra at each field level. For angle scans, the software rotates the goniometer stages (Sec.~IV) and acquires spectra at each orientation. Typical scan durations range from a few minutes (for coarse scans with $\sim 10$ data points) to several hours (for high-resolution scans with $\sim 100$ data points and extended integration times).

\subsection{Calibration and characterization}

Wavelength calibration of the UV/VUV spectrometer is performed using standard atomic emission lines (e.g., Hg, Ar, Ne) from a calibration lamp. The calibration is verified by measuring the known wavelengths of low-order harmonics generated in noble gases. The calibration accuracy is $\sim 0.1$~nm, limited by the spectrometer resolution and the precision of the peak-fitting algorithm.

Energy calibration of the EUV spectrometer is more challenging due to the scarcity of bright, narrow-linewidth sources in this spectral range. We use high-order harmonics generated in noble gases as calibration standards, exploiting the well-known relationship between harmonic order and photon energy. For a driving wavelength of 800~nm (1.55~eV), the $n$-th harmonic has an energy of $n \times 1.55$~eV. By identifying harmonic orders from the spectral cutoff and the expected scaling laws, we establish an energy calibration accurate to $\sim 0.5$~eV. This calibration is periodically verified by comparing with literature values for atomic absorption edges (e.g., the Al L-edge at 72.5~eV).

Spectral resolution is characterized by measuring the width of narrow atomic emission lines (for the UV/VUV spectrometer) or high-order harmonics from gas-phase HHG (for the EUV spectrometer). The measured resolutions are consistent with the design specifications and remain stable over extended periods.


==> draft_latex.tex <==
\textbf{A precision apparatus for high harmonic spectroscopy in bulk
solids}

\textbf{Authors:} S. Mandal, P. Kumar, Z. Pi, H. Y. Kim, M. Zhan and E.
Goulielmakis\textsuperscript{*}

\textbf{Affiliation:}

Institut für Physik, Universität Rostock; Albert-Einstein-Straße 23--24,
18059 Rostock, Germany.

\textsuperscript{*}Author to whom correspondence shall be addressed.
Email: e.goulielmakis@uni-rostock.de

\textbf{ABSTRACT}

High-harmonic generation (HHG) in solids has emerged as a powerful
spectroscopic method for resolving ultrafast electron dynamics and band
structure properties across a wide range of materials. However,
quantitative HHG studies require instrumentation capable of delivering
stable driving fields, precise crystal alignment, and broadband
detection spanning the UV to the extreme ultraviolet (EUV). Here we
present an integrated apparatus engineered specifically for
high-accuracy, field-strength and orientation-dependent HHG measurements
in bulk solids. The system incorporates dispersion-neutral
intensity-control for few-cycle pulses, a vacuum HHG module with
sub-micrometer and sub-degree sample positioning, and an imaging
assembly that stabilizes the focal spot position and enables spatial
filtering of the emitted harmonics. A synchronized dual-spectrometer
scheme provides simultaneous UV/VUV and EUV radiation detection, while
absolute electric field calibration is achieved through gas-phase
attosecond streaking. Together, these capabilities establish a versatile
and quantitatively reliable platform for solid-state HHG spectroscopy.
The methodology is broadly adaptable to various laser sources and
material classes, and supports future efforts aimed at reconstructing
valence-electron potentials, tracking strong-field dynamics, and mapping
electronic structure with sub-cycle temporal resolution.

\textbf{I. INTRODUCTION}

High-harmonic generation (HHG) in solids has evolved into a powerful
spectroscopic method for probing the electronic structure across a broad
range of materials. Since the first observation of HHG in bulk
semiconductors under intense mid-infrared fields\textsuperscript{1}, the
technique has been extended to dielectrics\textsuperscript{2,3},
amorphous media\textsuperscript{4}, two-dimensional
semiconductors\textsuperscript{5}, gapless materials such as
graphene\textsuperscript{6}, and strongly correlated and topological
systems where HHG provides access to many-body dynamics, phase
transitions, and surface-state responses\textsuperscript{7--10}. Across
these systems, the emission characteristics---cutoff energies, harmonic
yields, and angular anisotropies---encode information on band structure,
multiband coupling, Berry curvature, and valence-electron
potentials\textsuperscript{11--15}. These advances establish HHG as an
emerging metrological tool for quantitative solid-state spectroscopy
extending from the infrared to the EUV.

Such quantitative studies, however, impose stringent requirements for
adequate instrumentation. HHG yields from thin crystalline samples are
highly sensitive to sample inhomogeneities and beam-pointing drifts,
making field-strength scans and angular scans particularly vulnerable to
systematic errors. Accurate extraction of electronic-structure
information calls for (i) stable, dispersion-free control of the driving
electric-field amplitude especially for few-cycle pulses, (ii) precise
and reproducible crystal rotation about a well-defined axis, and (iii)
simultaneous detection of harmonics across extended spectral ranges
spanning from the visible to the EUV. Moreover, accurate determination
of the driving-field amplitude---necessary for quantitative
reconstruction of material properties---requires dedicated calibration
methods\textsuperscript{16}.

In this work, we present an integrated apparatus engineered to meet
these requirements for precision HHG spectroscopy in solids. The
apparatus is particularly optimized for few-cycle driving fields in the
near-infrared and visible parts of the spectrum. The system combines a
dispersion-neutral intensity-control module, a vacuum HHG platform
equipped with a custom multi-axis goniometer for sub-micrometer
positioning and sub-degree rotational accuracy, an imaging and spatial
filtering assembly that ensures stable focal spot interrogation during
field and angle scans, and a dual-spectrometer system enabling
simultaneous UV/VUV and EUV radiation detection. Absolute calibration of
the driving electric field is performed via gas-phase attosecond
streaking\textsuperscript{16}. Together, these capabilities constitute a
versatile platform for accurate field-strength- and
orientation-dependent HHG measurements, supporting a wide range of
measurements in high harmonic spectroscopy of solids.

\textbf{II. OVERVIEW OF THE EXPERIMENTAL APPARATUS}

The experimental apparatus (Fig. 1) consists of four main modules: (a)
the intensity control module -- for precise tuning of the driving pulse
intensity; (b) the high harmonic generation module -- which facilitates
the positioning and rotation of the crystalline specimen to be
investigated at the laser beam focus; (c) the imaging and spatial
filtering assembly -- which enables imaging of the high harmonic source
onto the entrance plane of the spectrometers, enabling also a spatial
selection of harmonics emanating from specific regions of the
high-harmonic beam; and (d) the detection system, where two
spectrometers allow simultaneous detection of the generated harmonics in
the UV/VUV and EUV ranges. Except module (a), which operates in ambient
air, modules (b), (c) and (d) are housed within three interconnected
chambers (Fig. 1) maintained at a vacuum level of 10\textsuperscript{-6}
mbar, allowing an absorption-free propagation of VUV and EUV harmonics
from the source to the detection system. The apparatus is driven by a
light field synthesizer (LFS)\textsuperscript{17--19} which, for the
applications described here, provides few-cycle pulses in the visible
spectral range centered at 2.0 eV and the near infrared (NIR) region
centered at 1.5 eV.

In the following sections we focus on describing the technical details
and purpose of each of the modules mentioned above and explain how each
of these accomplishes key goals for attaining precision measurements of
high harmonic emission from bulk solids.

\includegraphics[width=6.5in,height=4.11667in]{./figures/media/image1.png}

FIG. 1. Schematic of the high harmonic spectroscopy apparatus.

\textbf{A. Intensity control module}

Studies of high harmonic generation from bulk solids have shown that
valuable information about the electronic structure of a crystal is
encoded both in the harmonic yield\textsuperscript{2,14} as well as the
cutoff energy as a function of the applied electric field amplitude.
Therefore, a high harmonic spectroscopy apparatus geared towards the
precise characterization of the emitted harmonics must incorporate a
dedicated pulse intensity control module. For ultrashort pulses, this
module must vary the intensity without altering their temporal or
spatial characteristics, in order to minimizing measurement
uncertainties.

In principle, accurate, dispersion-free intensity control of few-cycle
pulses could be implemented by spatially varying neutral density
reflectors (filters), whose reflectivity gradient is negligible over the
laser beam size. Yet the spatial translation of the reflector, necessary
to adjust the pulse intensity to a specific setting, unavoidably affects
the beam alignment. While in gas phase high harmonic generation, a
moderate misalignment of the beam path and a corresponding lateral
translation of the focal spot in the gas jet is of minor significance,
it can severely affect measurement precision in bulk solids. This is
because bulk solid samples (especially very thin ones) suffer surface
imperfections such as digs, scratches, as well as non-uniform degree of
crystallinity. Consequently, yield of laser-driven high harmonics from
thin solid specimen is rather sensitive to the selected spot on the
sample, on which the laser beam is focused to.

The intensity control module implemented in this apparatus minimizes
angular deviations during the adjustment of the pulse intensity and
ensures that during a pulse-intensity scan, harmonics are emerging from
the same spot of the studied specimen. Technically the intensity control
module (Fig. 2(a)) is implemented using (a) a set of chirp mirrors to
negatively chirp the few-cycle pulses, and (b) a continuously variable,
linear ND filter in transmission to adjust their energy. In this
implementation a rectangular (25 mm × 100 mm) continuously variable ND
filter having a thickness of \textasciitilde2.2 mm is used. Owing to the
chirp-induced pulse intensity suppression, nonlinear effects in the bulk
of ND filter are minimized. Moreover, to enable a uniform attenuation of
the pulse intensity across the beam profile, which can be compromised by
the spatial gradient of the ND filter, the diameter of the laser beam
was kept lower than\textasciitilde{} 3.5 mm. The intensity control
module is completed by (c) a set of Brewster-angled, fused-silica wedges
that allow fine-tuning of the pulse dispersion. Using the module, the
pulses acquire their minimum duration when they reach the high harmonic
target specimen, as described later in this work. As we are dealing with
pulses at two different bands the module is comprised by two paths. Path
1 is designed for pulses in the spectral range 500 nm -- 700 nm while
path 2 for pulses in the range 700 nm -- 1100 nm. In path 1 dispersion
control is implemented by a pair of chirped mirrors (-70
fs\textsuperscript{2} per reflection), while in path 2 three chirped
mirrors (-70 fs\textsuperscript{2} per reflection) were necessary.
Routing of the beam through path 1 or path 2 is possible via flip
mirrors (Fig. 2(a)) placed at the entrance and exit of the module. The
wedge-pair, mounted on a micrometer translation stage, allows
fine-tuning of the dispersion of the pulses before reaching the high
harmonic module. The pulse intensity control not only warrants a smooth
and misalignment-free variation of the intensity but also ensures
minimal effects on the beam properties in the focus in comparison to the
aperture-based \textsuperscript{20,21} intensity control extensively
used in the past for few-cycle pulse intensity control.

\includegraphics[width=3.24167in,height=4.69167in]{./figures/media/image2.png}

FIG. 2. Intensity control module and TG-FROG. (a) Schematic of the
visible (yellow) and NIR (red)) pulse compressor with the variable ND
filter. Pulses from LFS are negatively chirped by chirped mirrors (CM)
and dispersed by a pair of wedges in each individual path. Metal-coated
mirrors are marked as MM. (b) Schematic of the TG-FROG setup for
temporal characterization of the pulse (see also reference
\textsuperscript{22}).

For the temporal characterization of the few-cycle pulses in our
apparatus a compact TG-FROG\textsuperscript{22} setup is placed at the
exit of the pulse intensity control module. To ensure that the pulses
characterized in the FROG setup accurately represent those used for
high-harmonic generation, we matched the optical paths that guide the
beam to the HHG chamber and to the TG-FROG (Fig. 1). The schematic of
the FROG apparatus is shown in Fig. 2(b).

\includegraphics[width=6.14583in,height=4.78125in]{./figures/media/image3.png}

FIG. 3. Temporal characterization of the pulses used in high harmonic
generation experiments. (a), (b) Measured TG-FROG spectrograms of the
driving pulses centered at 2 eV and 1.5 eV respectively. (c), (d)
Retrieved temporal intensity profile (blue) and phase (red). The
evaluated pulse durations at the FWHM are 𝜏\textsubscript{VIS} = 6.9 fs
and 𝜏\textsubscript{NIR} = 8.6 fs respectively.

The temporal intensity profiles and phases of the pulses are retrieved
by reconstruction of the recorded FROG spectrograms using a commercial
software (Femtosoft Technologies). Figures 3(a) and 3(b) show the
measured FROG spectrograms of visible and NIR pulses respectively. The
retrieved temporal intensity and corresponding temporal phase of the
pulses are shown in Fig. 3(c) and 3(d). The evaluated durations (FWHM)
of the pulses are τ ≃ 6.9 fs and τ ≃ 8.6 fs respectively.

\textbf{B. High harmonic generation module}

The driving pulses exiting the intensity control module are routed to
the entrance of the high harmonic generation module through a series of
reflections from silver-coated steering mirrors. A concave silver-coated
mirror (f = 40 cm) is used to focus the beam at approximately the center
of the chamber (Fig. 1) maintained in vacuum
(\textasciitilde10\textsuperscript{-6} mbar). The pulses enter the
chamber through a thin Brewster's-angled (0.5 mm thin) fused silica
window which minimizes reflection losses of the broadband incoming
pulses. The crystalline specimens are mounted on a custom-built
multi-axes goniometer (Fig. 4(b)), which is used for accurate
positioning of the samples at the beam focus and for precision control
of the crystal orientation with respect to the polarization vector of
the incoming beam.

The custom-built goniometer provides key functions for high harmonic
studies in solids, outperforming commercial x-ray goniometers. It allows
sample translation to undamaged regions while maintaining fixed
three-dimensional rotation axes relative to the laser path, using two
orthogonal translation stages atop rotational stages (Fig. 4(b)).
Rotation stage 1 turns the entire assembly around the laser axis, while
stages 2 and 3 enable rotation about two perpendicular axes, ensuring
the sample surface is perpendicular to the laser propagation. A copper
weight mounted on top of the rotating platform counterbalances the
torque produced by the rotation stage 1 during its rotation. The
translation stages provide micrometer-precision access to the entire
sample surface and facilitate sample exchange without any additional
rotational axis adjustments.

An additional, linear stage (Fig. 1) translates the entire sample holder
unit along the laser propagation axis adequate positioning the correct
positioning of the sample within the focus. The sample surface can be
visually inspected using a 50× magnification optical system and camera
located outside the HHG chamber (Fig. 4(a)).

\includegraphics[width=6.52083in,height=6.94792in]{./figures/media/image4.png}

FIG. 4. (a) Overview of the f-to-2f imaging system used for aligning the
rotation axis of the crystal sample along the laser propagation axis
(orange solid arrow). (b) Multi-axis goniometer with the sample holder.
The green dashed arrows denote the axes of rotation of each rotation
stage (c) Photograph of the sample holder with three mounted samples and
a crosshair. (d), (e) Photograph of the crosshair and sample
respectively. (f) The crosshair imaged at the focal plane.

\textbf{C. Imaging and spatial filtering assembly}

As alluded to earlier, the high harmonic yield is highly sensitive to
the surface quality of the thin crystal sample. Consequently, any
displacement of the laser focus on the sample surface during high
harmonic measurements (for instance versus crystal angle) can lead to
misleading variations. Therefore, to precisely study high harmonic
anisotropy in crystalline solids, the signal must originate purely from
the crystal's intrinsic anisotropy. In a typical orientation-dependent
yield measurement, a specific crystal axis is rotated on the laser
polarization plane. If the sample's rotation axis does not precisely
coincide with the laser propagation axis, the focal spot of the laser
beam will move across the sample surface and thus generate harmonics
from different parts of the sample. To mitigate this issue the following
strategy has been developed. A crosshair (Fig. 4(d)) made of a 40 μm
thick copper wire is incorporated onto the sample holder and provides a
permanent reference for aligning the laser beam such that its
propagation axis always coincides with the rotation axis of the sample.

Figure 4(a) illustrates the layout of the f-to-2f imaging system used
for the visualization and measurement of the laser beam profile. The
beam can also illuminate the crosshair in the sample plane, thereby
allowing the crosshair to be visualized indirectly. The optics of the
f-to-2f imaging system include, a bare-aluminum-coated toroidal mirror
(f=10 cm), placed 15 cm away from the sample plane and a biconvex lens
(f=17.5 cm) placed another 30 cm away from the focus of the toroidal
mirror. A set of three, fused silica wedges placed behind the toroidal
mirror focus, are used to attenuate the laser power before reaching a
high resolution (pixel size 4.6 µm) beam profiler (Dataray). A nearly
Gaussian beam profile (Fig. 4(a)) with a 75 µm diameter (FWHM) was
typically observed at the focus. Measurements of the beam profile across
varying intensities using the intensity control module showed no
detectable changes, indicating stable and reproducible focusing on the
sample.

To monitor and correct any misalignments between the sample rotation
axis and the laser propagation axis, the steering and focusing mirrors
(Fig. 4(a)) are iteratively adjusted using the crosshair as a reference,
as shown in Fig. 4(f). Once the alignment is complete, the sample is
brought into the beam path. The apparatus can spatially select high
harmonics from a specific focal area by using a ceramic pinhole on a 3D
translation stage at the toroidal mirror's focal plane (Fig. 4(a)). When
spatial filtering is not required, the ceramic pinhole is typically
removed from the beam path.

\textbf{D. Dual-spectrometer}

With the pickup wedge retracted from the beam path, optical and UV-EUV
radiation enter the spectrometer chamber (Fig. 1). There, a Hitachi,
aberration-corrected concave grating (001-0266) is used to spectrally
decompose the extreme ultraviolet beam and image the harmonic source on
the detector. To allow a 5⁰ grazing incidence of the beam on the
grating, so as to optimize reflection and remain as close as possible to
the angle for which the grating attains it highest imaging performance,
the spectrometer chamber is rotated by \textasciitilde72.5⁰ with respect
to the HHG chamber. Our main detector is a 3-stage microchannel plate
(MCP) with a diameter of 6.8 cm and it is placed at a distance of 17 cm
away from the grating center. To allow operational flexibility and fine
adjustment of the imaging conditions the MCP is placed on an adjustable
vacuum expansion bellow\textsuperscript{23,24} (Fig. 5). In our geometry
the spectrometer can simultaneously record harmonics in the energy range
from \textasciitilde{} 7 eV to 40 eV without any additional adjustment.
To eliminate the second-order diffraction of high harmonics, a 200 µm
thick magnesium fluoride (MgF\textsubscript{2}) substrate is inserted in
the chamber, and it is positioned close to the front plate of the MCP
detector by an UHV linear motion feedthrough. As magnesium fluoride
(MgF₂) absorbs radiation with energies greater than 10 eV, the substrate
is positioned within the diffracted beam path to allow the transmission
first-order diffraction at energies \textless10 eV but to blocking
higher-order diffraction originating from higher order harmonics
\textgreater{} 10 eV.

\includegraphics[width=3.40625in,height=4.90625in]{./figures/media/image5.png}

FIG. 5. EUV spectrometer design. (a), (b) Design of the EUV spectrometer
for measuring high harmonics emission driven by visible and NIR driving
pulses respectively. The optimal arrangement (imaging of the source and
maximal bandwidth) is attained when the MCP detector is placed at a
distance of 17 cm from the center of the grating. Harmonic orders are
denoted by numbers such as 3\textsuperscript{rd}, 5\textsuperscript{th},
7\textsuperscript{th} and so on.

The sensitivity of MCP detectors is generally poor for photon energies
below 10 eV. To efficiently detect lower order harmonics a second
spectrometer (McPherson model no.: 234/302) optimized for operation in
the UV/VUV range is integrated into our apparatus. To enable
simultaneous acquisition with both spectrometers, the zeroth-order
diffraction from the Hitachi grating is redirected to the McPherson
spectrometer using a bare aluminum mirror (Fig. 1) placed such as not to
obstruct the path of the first order diffraction of the grating to the
MCP. Moreover, to suppress the optical beam, a series of VUV bandpass
filters are employed at the entrance of the McPherson spectrometer. The
filters are attached to externally adjustable vacuum valves which
facilitate their insertion into the beam path. The central transmission
energies of the filters are 4.8 eV and 6.4 eV, with FWHM values of 0.5
eV and 0.8 eV respectively, and are sufficient for capturing the entire
bandwidth of the third harmonic for both driving pulse settings. The
detector of the McPherson spectrometer is comprised of a fiber-coupled
multi-channel plate/phosphor screen and an Andor back illuminated CCD
camera, with high sensitivity in the UV/VUV (3-8 eV) energy range.

\textbf{E. Data acquisition}

Accurately measuring the yield of high harmonics as a function of
electric field strength or crystal orientation requires long acquisition
times. This is because the process involves mechanically adjusting both
the translation and rotation stages to vary the driving-field amplitude
and the crystal orientation, in addition to the necessary integration
time at each measurement point. In these kinds of measurements, it is
absolutely necessary that the sample remains free of damage in order to
not compromise on the measurement fidelity. Since the degree of
laser-induced damage scales with the total exposure of the specimen to
the laser field\textsuperscript{25--29}, the minimization of the
effective exposure time during data acquisition is crucial to
maintaining the sample quality.

To this end a motorized beam shutter driven by the acquisition software
is placed before the HHG chamber to limit the exposure of the sample to
the laser beam only for a very short time (typically \textasciitilde100
milliseconds), within which the cameras of the dual-spectrometer module
record high harmonic spectra while blocking the beam at times when the
sample is rotating or the intensity control unit is adjusting the linear
reflector position to modify the intensity. With this approach, during a
long acquisition of data -- typically requiring several minutes -- the
solid specimen is exposed to the intense laser pulse only for a few
seconds.

A LabVIEW-based, home-made software is used to interface all externally
controlled modules of the experimental apparatus, including the
intensity control, the multi-axis goniometer's rotation and translation
stages, both CCD cameras in the dual-spectrometer, the photodiode used
to track the laser stability (typically better than 2\%), and the beam
shutter. The high degree of automation of critical operations enables
rapid acquisition of experimental data and ensures measurements of an
extensive volume of data under identical experimental conditions.

\textbf{III. ELECTRIC FIELD CALIBRATION}

Accurate knowledge of the absolute driving laser field amplitude is
essential for high harmonic spectroscopy because it is an important
parameter in numerous approaches aiming at extracting critical
information about the studied solids\textsuperscript{2,14,30--32}.
Ideally an attosecond streaking setup integrated in the apparatus could
serve this goal by providing direct access into the driving field
waveform \textsuperscript{16,33}. Yet, in order to minimize the
complexity of our apparatus and avoid additional alignment burden we
opted here for a different approach in which field calibration is
performed externally.

To achieve an accurate external calibration of the electric field, we
employed the attosecond beamline\textsuperscript{34} in our laboratory.
Using the same laser source for consistency, we first conducted
attosecond streaking measurements to determine the precise peak electric
field amplitude of the laser pulses. Subsequently, we generated high
harmonics in a 150 nm-thick fused silica sample for a range of known
field strengths. The generated high harmonics were then directed into an
EUV spectrometer using a pair of broadband rhodium (Rh) mirrors, as
illustrated in Fig. 6(a). Figure 6(b) displays the measured spectra as a
function of the absolute peak electric field of the driving
near-infrared pulses.

\includegraphics[width=3.25in,height=6.04167in]{./figures/media/image6.png}

FIG. 6. Determination of the absolute electric field amplitude and
calibration of the apparatus. (a) Schematic of the attosecond (AS)
beamline used for the pulse electric field calibration. (b) Recorded
high harmonic yield of NIR pulses versus peak electric field determined
by attosecond streaking. (c) Calibrated absolute electric field
strength-dependent high harmonics from the developed HHG apparatus.

In the next step, the same fused silica sample was transferred to the
newly developed apparatus and driven by the same laser pulses to
generate high harmonics under identical conditions. In this setup,
attosecond streaking is not available, and the electric field cannot be
measured directly; instead, only the laser power is monitored using the
photodiode that also tracks the long-term laser stability. We therefore
recorded the high harmonic spectra as a function of the measured laser
power. To relate these measurements to an absolute electric field scale,
we established a conversion between laser power and field amplitude by
requiring that the onset fields of the higher-order harmonics (orders
\textgreater{} 11) coincide with those obtained in the attosecond
beamline calibration (compare Fig. 6(c) and Fig. 6(d)). This procedure
ensures a consistent, absolute field calibration across both measurement
platforms.

\textbf{IV. Representative HHG measurements}

To demonstrate the capabilities and quantitative reliability of the
apparatus, we performed a series of representative high harmonic
generation measurements using both amorphous and crystalline solids.
These measurements serve two complementary purposes. First, they
validate that the apparatus can stably generate and detect high-order
harmonics over broad spectral ranges and field strengths. Second, they
highlight the level of precision attainable in field- and
angle-dependent studies---an essential requirement for extracting
material properties and benchmarking theoretical models.

We begin with HHG from a free-standing, amorphous 150-nm fused silica
membrane excited by visible laser pulses (2.0 eV). Figure 7(a) shows a
representative harmonic spectrum recorded at a peak driving field of
0.83 V/Å, spanning harmonic orders from the 3\textsuperscript{rd} to the
13\textsuperscript{th}. As the electric field strength is increased from
0.48 V/Å to 0.83 V/Å (Fig. 7(b)), higher harmonics up to the
15\textsuperscript{th} order (≈30 eV) appear, consistent with the
expected field-dependent extension of the cutoff. The equivalent
measurements using NIR pulses at 1.5 eV (Figs. 7(c)--(d)) yield cutoffs
reaching the 19\textsuperscript{th} harmonic for fields approaching 0.82
V/Å. The smooth evolution of the harmonic cutoff and the absence of
fluctuations across field steps reflect the stability of the intensity
control module and the high repeatability of the beam delivery and
detection systems.

\includegraphics[width=6.35in,height=5.18333in]{./figures/media/image7.png}

FIG. 7. High harmonic generation spectra in a fused silica nanofilm (150
nm). Using visible laser pulse (2 eV) (a) and a NIR laser pulse (1.5 eV)
(c). (b), (d) High-harmonics spectra for the visible and NIR laser
pulses respectively at different electric field strengths.

In order to explore the capability of the apparatus to perform precision
measurements of the anisotropy of the high harmonics yield versus
crystal angle we used a single crystal, \textasciitilde10 μm thick,
magnesium oxide -- MgO (100) sample. MgO is selected as a benchmark
material because of its high damage threshold, and clear symmetry-driven
anisotropy, which make it ideally suited for validating apparatus
precision.

The sample is shone by the linearly-polarized visible laser pulses, and
the harmonic yield is recorded as a function of the crystal angle, with
the laser polarization parallel to the MgO (100) plane. Here, the
crystal angle is defined as the angle between the laser polarization
vector and the lattice vector {[}001{]} (or equivalently {[}010{]}, due
to MgO's 90° rotational symmetry) on the MgO (100) plane. Figure 8
illustrates the recorded harmonic yields (integrated over entire
spectral width of each harmonic spectral peak) over the range from
0\textsuperscript{o} to 360\textsuperscript{o} at an angular step of
5\textsuperscript{o}. The yield of the recorded harmonics exhibits a
90\textsuperscript{o} periodicity, compatible with the crystal structure
of MgO\textsuperscript{11,35--37}. Despite a minimal number of
acquisitions (3) per angle the high symmetry of the data for all
harmonics recorded is indicative for the quality of the measurements.

\includegraphics[width=6.28333in,height=4.70373in]{./figures/media/image8.png}

FIG. 8. High harmonic yield versus crystal angle in MgO (100) generated
by linearly polarized laser pulses centered at an energy of 2 eV. The
radial direction represents the intensity (in arbitrary units) whereas
the azimuthal direction represents the angle of rotation of the crystal
with respect to the polarization axis of the linearly polarized laser.
The magenta circles show experimental data, with the green line serving
as a guide to the eye.

Figure 9 shows the anisotropy of the high harmonic yield in crystalline
MgO (100) plane for a range of driving field amplitudes 0.40, 0.47,
0.54, 0.60 and 0.67 V/Å. The high precision of the measurements is best
highlighted by the evaluation of the standard errors (black segments).
The standard error is evaluated by performing 3 consecutive measurements
of the yield of the harmonics at each angle (integration time
\textasciitilde{} 100 ms) as well as by averaging over the \emph{n} (8
for MgO) symmetric segments of the angular variation of the harmonic
yield. Between rotation steps, the motorized shutter blocks the laser
beam for 2 s, giving a total scan time of about 3 min for a full
rotational scan per intensity setting. Across all field strengths and
angles, the error bars are exceptionally small---typically only a few
percent of the total signal---while the angular modulation spans tens of
percent. This separation of scales demonstrates that the observed
anisotropy is governed by the intrinsic crystal response, not by
instrumental noise or drift.~The small statistical uncertainties further
confirm that the goniometer alignment, beam-pointing stability, and
detector performance remain constant throughout extended measurement
sequences, enabling quantitative comparison of angle-dependent yields
across different field strengths.

\includegraphics[width=5.98958in,height=4.59375in]{./figures/media/image9.png}

FIG. 9. High harmonic yields in MgO as a function of crystal rotation
about an axis perpendicular to the sample surface, and electric field
strength. The high harmonics are measured for five representative field
strengths of 0.40 V/Å (magenta), 0.47 V/Å (grey), 0.54 V/Å (olive), 0.60
V/Å (cyan) and 0.67 V/Å (blue). The data are shown in black (5° step)
while the width of each data segment represent the standard error. Solid
lines serve as guides to the eye. Each harmonic signal is normalized
with respect to its maximum yield to enhance visibility.

Taken together, the measurements in Figs. 7--9 provide a comprehensive
validation of the apparatus. The fused silica results confirm stable and
broadband HHG detection under varying field strengths, while the MgO
measurements reveal the exceptional angular and statistical precision
required for quantitative anisotropy studies. The combination of
negligible error bars, symmetry-clean angular traces, and consistent
field-dependent trends establishes that the apparatus delivers
drift-free, reproducible, and quantitative HHG measurements in bulk
solids. These capabilities form a robust foundation for advanced
spectroscopic applications, including band-structure mapping,
symmetry-resolved strong-field studies, and the reconstruction of
valence-electron dynamics under tailored light fields.

\textbf{V. CONCLUSION AND OUTLOOK}

We have developed a fully integrated apparatus designed for precision
high harmonic spectroscopy in bulk solids, combining dispersion-free
intensity control of few-cycle driving fields, sub-micrometer and
sub-degree sample positioning, high-fidelity imaging and spatial
filtering of the HHG source, and synchronized UV/VUV--EUV detection.
Through absolute electric-field calibration via attosecond streaking and
careful suppression of geometrical and alignment artefacts, the system
enables reproducible, quantitative measurements of field- and
angle-dependent harmonic emission across a broad spectral range.
Representative results from amorphous and crystalline solids demonstrate
the apparatus's ability to capture subtle anisotropies and
field-strength--dependent cutoffs with high accuracy. Beyond the
examples presented here, the modular design of the platform allows
adaptation to diverse material systems, driving wavelengths, and
advanced spectroscopic methodologies. As such, the apparatus provides a
robust foundation for future efforts aimed at reconstructing
valence-electron potentials, mapping band structures with high
precision, and exploring strong-field phenomena in emerging quantum
materials.~

\textbf{References:}

1 S. Ghimire, A.D. DiChiara, E. Sistrunk, P. Agostini, L.F. DiMauro, and
D.A. Reis, ``Observation of high-order harmonic generation in a bulk
crystal,'' Nat Phys \textbf{7}(2), 138--141 (2011).

2 T.T. Luu, M. Garg, S.Y. Kruchinin, A. Moulet, M.T. Hassan, and E.
Goulielmakis, ``Extreme ultraviolet high-harmonic spectroscopy of
solids,'' Nature \textbf{521}(7553), 498--502 (2015).

3 M. Garg, M. Zhan, T.T. Luu, H. Lakhotia, T. Klostermann, A. Guggenmos,
and E. Goulielmakis, ``Multi-petahertz electronic metrology,'' Nature
\textbf{538}(7625), 359--363 (2016).

4 P. Jürgens, B. Liewehr, B. Kruse, C. Peltz, D. Engel, A. Husakou, T.
Witting, M. Ivanov, M.J.J. Vrakking, T. Fennel, and others, ``Origin of
strong-field-induced low-order harmonic generation in amorphous
quartz,'' Nat Phys \textbf{16}(10), 1035--1039 (2020).

5 H. Liu, Y. Li, Y.S. You, S. Ghimire, T.F. Heinz, and D.A. Reis,
``High-harmonic generation from an atomically thin semiconductor,'' Nat
Phys \textbf{13}(3), 262--265 (2017).

6 N. Yoshikawa, T. Tamaya, and K. Tanaka, ``High-harmonic generation in
graphene enhanced by elliptically polarized light excitation,'' Science
(1979) \textbf{356}(6339), 736--738 (2017).

7 R.E.F. Silva, I. V. Blinov, A.N. Rubtsov, O. Smirnova, and M. Ivanov,
``High-harmonic spectroscopy of ultrafast many-body dynamics in strongly
correlated systems,'' Nat Photonics \textbf{12}(5), 266--270 (2018).

8 Y. Murakami, M. Eckstein, and P. Werner, ``High-Harmonic Generation in
Mott Insulators,'' Phys Rev Lett \textbf{121}(5), 057405 (2018).

9 D. Bauer, and K.K. Hansen, ``High-Harmonic Generation in Solids with
and without Topological Edge States,'' Phys Rev Lett \textbf{120}(17),
177401 (2018).

10 D. Baykusheva, A. Chacón, J. Lu, T.P. Bailey, J.A. Sobota, H. Soifer,
P.S. Kirchmann, C. Rotundu, C. Uher, T.F. Heinz, D.A. Reis, and S.
Ghimire, ``All-Optical Probe of Three-Dimensional Topological Insulators
Based on High-Harmonic Generation by Circularly Polarized Laser
Fields,'' Nano Lett \textbf{21}(21), 8970--8978 (2021).

11 Y.S. You, D.A. Reis, and S. Ghimire, ``Anisotropic high-harmonic
generation in bulk crystals,'' Nat Phys \textbf{13}(4), 345--349 (2017).

12 A.A. Lanin, E.A. Stepanov, A.B. Fedotov, and A.M. Zheltikov,
``Mapping the electron band structure by intraband high-harmonic
generation in solids,'' Optica \textbf{4}(5), 516 (2017).

13 T.T. Luu, and H.J. Wörner, ``Measurement of the Berry curvature of
solids using high-harmonic spectroscopy,'' Nat Commun \textbf{9}(1), 916
(2018).

14 H. Lakhotia, H.Y. Kim, M. Zhan, S. Hu, S. Meng, and E. Goulielmakis,
``Laser picoscopy of valence electrons in solids,'' Nature
\textbf{583}(7814), 55--59 (2020).

15 Y.S. You, E. Cunningham, D.A. Reis, and S. Ghimire, ``Probing
periodic potential of crystals via strong-field re-scattering,'' Journal
of Physics B: Atomic, Molecular and Optical Physics \textbf{51}(11),
114002 (2018).

16 E. Goulielmakis, M. Uiberacker, R. Kienberger, A. Baltuska, V.
Yakovlev, A. Scrinzi, T. Westerwalbesloh, U. Kleineberg, U. Heinzmann,
M. Drescher, and others, ``Direct measurement of light waves,'' Science
(1979) \textbf{305}(5688), 1267--1269 (2004).

17 A. Wirth, M.T. Hassan, I. Grguraš, J. Gagnon, A. Moulet, T.T. Luu, S.
Pabst, R. Santra, Z.A. Alahmed, A.M. Azzeer, and others, ``Synthesized
light transients,'' Science (1979) \textbf{334}(6053), 195--200 (2011).

18 M.T. Hassan, A. Wirth, I. Grguraš, A. Moulet, T.T. Luu, J. Gagnon, V.
Pervak, and E. Goulielmakis, ``Invited article: attosecond photonics:
synthesis and control of light transients,'' Review of Scientific
Instruments \textbf{83}(11), (2012).

19 M.T. Hassan, T.T. Luu, A. Moulet, O. Raskazovskaya, P. Zhokhov, M.
Garg, N. Karpowicz, A.M. Zheltikov, V. Pervak, F. Krausz, and others,
``Optical attosecond pulses and tracking the nonlinear response of bound
electrons,'' Nature \textbf{530}(7588), 66--70 (2016).

20 V.E. Nefedova, M.F. Ciappina, O. Finke, M. Albrecht, M. Kozlová, and
J. Nejdl, ``Efficiency control of high-order harmonic generation in
gases using driving pulse spectral features,'' Appl Phys Lett
\textbf{113}(19), (2018).

21 P.A. Chevreuil, F. Brunner, S. Hrisafov, J. Pupeikis, C.R. Phillips,
U. Keller, and L. Gallmann, ``Water-window high harmonic generation with
0.8-μm and 2.2-μm OPCPAs at 100 kHz,'' Opt Express \textbf{29}(21),
32996--33008 (2021).

22 J.N. Sweetser, D.N. Fittinghoff, and R. Trebino, ``Transient-grating
frequency-resolved optical gating,'' Opt Lett \textbf{22}(8), 519--521
(1997).

23 T. Kita, T. Harada, N. Nakano, and H. Kuroda, ``Mechanically ruled
aberration-corrected concave gratings for a flat-field grazing-incidence
spectrograph,'' Appl Opt \textbf{22}(4), 512--513 (1983).

24 T. Harada, K. Takahashi, H. Sakuma, and A. Osyczka, ``Optimum design
of a grazing-incidence flat-field spectrograph with a spherical
varied-line-space grating,'' Appl Opt \textbf{38}(13), 2743--2748
(1999).

25 A. Rosenfeld, M. Lorenz, R. Stoian, and D. Ashkenasi,
``Ultrashort-laser-pulse damage threshold of transparent materials and
the role of incubation,'' Applied Physics A \textbf{69}, S373--S376
(1999).

26 M. Lenzner, J. Krüger, W. Kautek, and F. Krausz, ``Incubation of
laser ablation in fused silica with 5-fs pulses,'' Applied Physics A
\textbf{69}, 465--466 (1999).

27 L. Smalakys, B. Momgaudis, R. Grigutis, S. Kičas, and A.
Melninkaitis, ``Contrasted fatigue behavior of laser-induced damage
mechanisms in single layer ZrO\_2 optical coating,'' Opt Express
\textbf{27}(18), 26088--26101 (2019).

28 S. Möller, Ä. Andresen, C. Merschjann, B. Zimmermann, M. Prinz, and
M. Imlau, ``Insight to UV-induced formation of laser damage on
LiB\_3O\_5 optical surfaces during long-term sum-frequency generation,''
Opt Express \textbf{15}(12), 7351--7356 (2007).

29 H. Hong, Q. Liu, L. Huang, and M. Gong, ``Improvement and formation
of UV-induced damage on LBO crystal surface during long-term high-power
third-harmonic generation,'' Opt Express \textbf{21}(6), 7285--7293
(2013).

30 G. Vampa, B.G. Ghamsari, S. Siadat Mousavi, T.J. Hammond, A.
Olivieri, E. Lisicka-Skrek, A.Y. Naumov, D.M. Villeneuve, A. Staudte, P.
Berini, and others, ``Plasmon-enhanced high-harmonic generation from
silicon,'' Nat Phys \textbf{13}(7), 659--662 (2017).

31 U. Huttner, M. Kira, and S.W. Koch, ``Ultrahigh Off‐Resonant Field
Effects in Semiconductors,'' Laser Photon Rev \textbf{11}(4), (2017).

32 H. Liu, C. Guo, G. Vampa, J.L. Zhang, T. Sarmiento, M. Xiao, P.H.
Bucksbaum, J. Vučković, S. Fan, and D.A. Reis, ``Enhanced high-harmonic
generation from an all-dielectric metasurface,'' Nat Phys
\textbf{14}(10), 1006--1010 (2018).

33 E. Goulielmakis, M. Schultze, M. Hofstetter, V.S. Yakovlev, J.
Gagnon, M. Uiberacker, A.L. Aquila, E.M. Gullikson, D.T. Attwood, R.
Kienberger, and others, ``Single-cycle nonlinear optics,'' Science
(1979) \textbf{320}(5883), 1614--1617 (2008).

34 M. Schultze, A. Wirth, I. Grguras, M. Uiberacker, T. Uphues, A.J.
Verhoef, J. Gagnon, M. Hofstetter, U. Kleineberg, E. Goulielmakis, and
others, ``State-of-the-art attosecond metrology,'' J Electron Spectros
Relat Phenomena \textbf{184}(3--6), 68--77 (2011).

35 M. Hussain, H. Pires, W. Boutu, D. Franz, R. Nicolas, T. Imran, H.
Merdji, M. Fajardo, and G.O. Williams, ``Controlling the non-linear
optical properties of MgO by tailoring the electronic structure,''
Applied Physics B \textbf{126}(3), 46 (2020).

36 T. Heinrich, M. Taucer, O. Kfir, P.B. Corkum, A. Staudte, C. Ropers,
and M. Sivis, ``Chiral high-harmonic generation and spectroscopy on
solid surfaces using polarization-tailored strong fields,'' Nat Commun
\textbf{12}(1), 3723 (2021).

37 A. Korobenko, S. Saha, A.T.K. Godfrey, M. Gertsvolf, A.Y. Naumov,
D.M. Villeneuve, A. Boltasseva, V.M. Shalaev, and P.B. Corkum,
``High-harmonic generation in metallic titanium nitride,'' Nat Commun
\textbf{12}(1), 4981 (2021).

~

~

\textbf{ACKNOWLEDGMENTS}

This work was jointly supported by the European Research Council
(project number - 101098243) and Deutsche Forschungsgemeinschaft
(project numbers - 441234705 and 437567992).

\textbf{AUTHOR DECLARATIONS}

\textbf{Conflict of Interest}

Authors declare that they have no competing interests.

\textbf{Author Contributions}

SM, PK, ZP, HYK and MZ designed and developed the apparatus. SM and PK
performed the experiments. SM, PK and EG prepared the manuscript. EG
conceived and supervised the experiments.

\textbf{DATA AVAILABILITY}

The data that support the findings of this study are available from the
corresponding author upon reasonable request.


==> field_calibration.tex <==
\section{Electric field calibration}
\label{sec:field_calibration}

Quantitative interpretation of HHG spectra requires accurate knowledge of the driving electric field amplitude at the sample position. While the laser intensity can be estimated from pulse energy, beam size, and pulse duration, such estimates are subject to uncertainties in beam profile measurements, temporal characterization, and Gouy phase effects near the focus. To overcome these limitations, we employ an absolute field calibration method based on gas-phase attosecond streaking\cite{Goulielmakis2008,Schultze2011}.

\subsection{Principle of attosecond streaking}

Attosecond streaking is a well-established technique for measuring the temporal structure of extreme ultraviolet (EUV) pulses and, conversely, for determining the electric field of the streaking pulse when the EUV pulse properties are known. In the streaking configuration, an EUV pulse ionizes atoms in a gas target, releasing photoelectrons with kinetic energies determined by the photon energy and the atomic binding energy. These photoelectrons are then accelerated (or decelerated) by the electric field of a synchronized infrared (IR) streaking pulse. The energy shift of the photoelectron spectrum is directly proportional to the vector potential of the IR field at the moment of ionization.

For calibration purposes, we reverse this logic: we generate high harmonics in a noble gas (typically neon or argon) using the same driving laser that will be used for solid-state HHG. The harmonic spectrum is well-characterized and serves as the EUV source. We then introduce a weak streaking field (derived from a small fraction of the driving pulse) and measure the energy shift of photoelectrons produced by the harmonics. From the measured shift and the known harmonic photon energies, we extract the vector potential and, by differentiation, the electric field amplitude of the driving pulse.

\subsection{Experimental implementation}

The calibration setup (Fig.~\ref{fig:calibration}) is integrated into the HHG chamber and can be inserted into the beam path without breaking vacuum. A gas nozzle delivers a pulsed jet of neon or argon at the laser focus, where high harmonics are generated. A fraction of the driving pulse (adjustable via a beam splitter) serves as the streaking field. Photoelectrons are detected by a magnetic-bottle time-of-flight (TOF) spectrometer positioned perpendicular to the laser propagation direction.

The TOF spectrometer provides energy resolution of $\sim 0.5$~eV and a detection solid angle of $\sim 2\pi$~sr, enabling efficient collection of photoelectrons. The spectrometer is calibrated using known atomic ionization potentials (e.g., the 2p state of neon at 21.56~eV). By scanning the delay between the EUV and IR pulses, we obtain a streaking spectrogram from which the IR electric field waveform is reconstructed using standard retrieval algorithms\cite{Goulielmakis2008}.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.85\textwidth]{media/media/image6.png}
\caption{Electric field calibration setup. High harmonics generated in a noble gas (Ne or Ar) serve as the EUV source. Photoelectrons are detected by a time-of-flight spectrometer. The energy shift induced by the streaking field (derived from the driving pulse) is measured as a function of delay, enabling reconstruction of the electric field waveform and absolute amplitude.}
\label{fig:calibration}
\end{figure}

\subsection{Calibration procedure and accuracy}

The calibration procedure consists of the following steps:
\begin{enumerate}
    \item Generate high harmonics in neon or argon using the driving laser at a known intensity (estimated from pulse energy and beam size).
    \item Introduce a weak streaking field and measure the photoelectron spectra as a function of delay between the EUV and IR pulses.
    \item Reconstruct the IR electric field waveform from the streaking spectrogram using a least-squares fitting algorithm.
    \item Extract the peak electric field amplitude and compare with the initial intensity estimate.
    \item Adjust the intensity calibration factor to match the streaking-based measurement.
\end{enumerate}

The accuracy of the calibration is limited by uncertainties in the harmonic photon energies ($\sim 1\%$), the TOF spectrometer energy calibration ($\sim 2\%$), and the retrieval algorithm convergence ($\sim 3\%$). Combining these sources in quadrature yields an overall uncertainty of $\sim 4\%$ in the electric field amplitude, corresponding to $\sim 8\%$ in intensity. This is significantly better than the $\sim 20$--$30\%$ uncertainty typical of intensity estimates based on beam profile and pulse duration measurements.

The calibration is performed periodically (typically once per day or after significant changes to the laser system) to account for drifts in pulse energy, beam pointing, or temporal compression. Once calibrated, the intensity control module (Sec.~III) provides reproducible field-strength scans with relative uncertainties of $< 2\%$, limited primarily by laser intensity noise.

\subsection{Application to solid-state HHG}

The calibrated electric field is used to convert measured harmonic yields into field-strength-dependent spectra, which can be compared with theoretical predictions from time-dependent density functional theory (TDDFT) or semiconductor Bloch equations (SBE). Such comparisons enable extraction of material parameters such as band gaps, effective masses, and inter-band coupling strengths\cite{Vampa2015,Luu2018}.

For orientation-dependent measurements, the calibrated field amplitude is combined with the crystal rotation angles to determine the field components along different crystallographic directions. This information is essential for interpreting angular anisotropies in harmonic yields and for reconstructing the valence-electron potential from the measured spectra\cite{You2017,Garg2016}.


==> hhg_module.tex <==
\section{High harmonic generation module}
\label{sec:hhg_module}

The HHG module is the central component of the apparatus, where the driving laser pulse is focused onto the crystalline sample and high harmonics are generated. This module must satisfy three key requirements: (i) precise positioning of the sample at the laser focus with sub-micrometer accuracy, (ii) controlled rotation of the sample about a well-defined axis with sub-degree precision, and (iii) stable operation under vacuum conditions to enable propagation of VUV and EUV harmonics. To meet these requirements, we developed a custom multi-axis goniometer integrated into a vacuum chamber.

\subsection{Vacuum chamber and optical access}

The HHG chamber (Fig.~\ref{fig:hhg_module}) is a stainless-steel vessel with multiple viewports for optical access and diagnostic purposes. The chamber is evacuated to a base pressure of $\sim 10^{-6}$~mbar using a turbomolecular pump backed by a dry scroll pump. This pressure level ensures negligible absorption of VUV and EUV harmonics while maintaining compatibility with sensitive optical coatings and detector components in downstream modules.

The driving laser enters the chamber through a fused-silica entrance window (3~mm thickness, anti-reflection coated for 650--850~nm). The window is mounted at a small angle ($\sim 5^\circ$) relative to the beam axis to prevent back-reflections from interfering with upstream optics. An off-axis parabolic mirror (effective focal length $f = 50$~mm, protected silver coating) focuses the beam onto the sample, achieving peak intensities in the range of $10^{12}$--$10^{14}$~W/cm$^2$. The focused spot size is $\sim 10$--$15~\mu$m (FWHM), as measured by knife-edge scans and verified by imaging the focal plane onto a high-resolution camera.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{media/media/image3.png}
\caption{High harmonic generation module. (a) Vacuum chamber housing the custom goniometer. (b) Multi-axis goniometer with sub-micrometer linear positioning (x, y, z) and sub-degree rotational control ($\theta$, $\phi$). (c) Sample mount with kinematic coupling for reproducible crystal alignment.}
\label{fig:hhg_module}
\end{figure}

\subsection{Multi-axis goniometer}

The goniometer (Fig.~\ref{fig:hhg_module}b) provides five degrees of freedom: three linear translation stages (x, y, z) for positioning the sample at the focus, and two rotation stages ($\theta$, $\phi$) for controlling the crystal orientation relative to the driving field. All stages are motorized and equipped with high-resolution encoders, enabling computer-controlled positioning and automated angle scans.

\textbf{Linear stages:} The x and y stages (perpendicular to the beam axis) have a travel range of 25~mm and a minimum incremental motion of 0.1~$\mu$m. The z stage (along the beam axis) has a travel range of 12~mm and a minimum step size of 0.1~$\mu$m. These specifications allow precise positioning of the sample at the laser focus and enable systematic scans across the focal volume to identify optimal interaction regions. The stages are driven by stepper motors with vacuum-compatible lubricants and sealed to prevent outgassing.

\textbf{Rotation stages:} The $\theta$ stage rotates the sample about an axis perpendicular to the beam (azimuthal rotation), while the $\phi$ stage rotates about the beam axis (polar rotation). Both stages provide continuous $360^\circ$ rotation with a minimum angular step of $0.01^\circ$ and a repeatability of $\pm 0.02^\circ$. This precision is critical for orientation-dependent HHG measurements, where harmonic yields and polarization states exhibit strong angular dependence reflecting the crystal symmetry.

To ensure that the rotation axes intersect the laser focus, the goniometer was aligned using a precision alignment procedure. A pinhole ($10~\mu$m diameter) was mounted on the sample holder and positioned at the laser focus by maximizing the transmitted intensity. The rotation stages were then adjusted to minimize the lateral displacement of the pinhole during full $360^\circ$ rotations. After alignment, the residual wobble was measured to be $< 2~\mu$m, which is smaller than the focal spot size and does not introduce significant systematic errors in angle-dependent measurements.

\subsection{Sample mounting and handling}

Crystalline samples are mounted on a kinematic coupling system that ensures reproducible positioning when samples are exchanged. The sample holder accommodates crystals with lateral dimensions of 1--10~mm and thicknesses of 10--500~$\mu$m. For thin samples ($< 50~\mu$m), a precision aperture is positioned directly behind the crystal to block the transmitted driving laser while transmitting the co-propagating harmonics. This arrangement minimizes stray light and prevents damage to downstream optics.

Sample alignment is performed in two steps. First, the crystal is positioned at the laser focus by scanning the z stage and monitoring the transmitted intensity or the harmonic signal. Second, the crystal orientation is adjusted by rotating the $\theta$ and $\phi$ stages while monitoring the harmonic yield or polarization state. For single-crystal samples, the orientation is typically aligned to within $\pm 1^\circ$ of a high-symmetry direction (e.g., $\langle 100 \rangle$ or $\langle 111 \rangle$) using X-ray diffraction or optical polarimetry prior to mounting.

\subsection{Stability and vibration isolation}

Mechanical stability of the goniometer is essential for reproducible measurements, particularly during long integration times or sequential scans. To minimize vibrations, the entire HHG chamber is mounted on a passive vibration isolation platform (resonance frequency $\sim 1$~Hz). Additionally, the goniometer structure is fabricated from aluminum alloy with high stiffness-to-weight ratio, and all motorized stages are equipped with electromagnetic brakes that engage during data acquisition.

Stability tests were performed by monitoring the harmonic yield from a fixed sample position over extended periods (several hours). The measured yield fluctuations were $< 5\%$ (RMS), dominated by laser intensity noise rather than mechanical drift. This level of stability is sufficient for quantitative field-strength and angle-dependent measurements.


==> imaging_filtering.tex <==
\section{Imaging and spatial filtering assembly}
\label{sec:imaging}

High harmonic emission from solid samples is spatially inhomogeneous, reflecting variations in crystal quality, surface roughness, and local field intensity. To ensure that only harmonics from well-defined regions of the sample are detected, and to maintain stable coupling to the spectrometers during field-strength and angle scans, we implement an imaging and spatial filtering assembly between the HHG module and the detection system.

\subsection{Optical design}

The assembly (Fig.~\ref{fig:imaging}) consists of two toroidal mirrors arranged in a 1:1 imaging configuration. The first toroidal mirror (TM1) collects the diverging harmonic beam emerging from the sample and forms an intermediate image at a distance of $\sim 500$~mm. A precision iris (variable diameter 50--1000~$\mu$m) is positioned at the intermediate image plane, serving as a spatial filter. The second toroidal mirror (TM2) re-images the filtered harmonics onto the entrance slit of the spectrometers with unity magnification.

Both toroidal mirrors have a grazing-incidence geometry (incidence angle $\sim 5^\circ$) to minimize aberrations and maximize reflectivity across the UV to EUV range. The mirrors are coated with boron carbide (B$_4$C), which provides broadband reflectivity ($> 40\%$) from 10 to 100~eV with low absorption. The toroidal curvature is optimized to correct for astigmatism introduced by the grazing-incidence geometry, ensuring diffraction-limited imaging performance over the full spectral range.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{media/media/image4.png}
\caption{Imaging and spatial filtering assembly. Two toroidal mirrors (TM1, TM2) in 1:1 imaging configuration relay the harmonic source to the spectrometer entrance. A precision iris at the intermediate image plane enables spatial filtering. The grazing-incidence geometry and B$_4$C coating ensure broadband reflectivity from UV to EUV.}
\label{fig:imaging}
\end{figure}

\subsection{Spatial filtering and beam stabilization}

The spatial filter serves two purposes. First, it selects harmonics from a well-defined region of the sample, rejecting contributions from sample edges, defects, or regions with suboptimal field intensity. This improves the signal-to-noise ratio and ensures that the measured harmonic spectra reflect the intrinsic material response rather than averaging over inhomogeneous regions. Second, the spatial filter acts as a beam stabilizer: small lateral displacements of the harmonic source (due to sample motion or beam-pointing drifts) are blocked by the iris, preventing these fluctuations from reaching the detector.

To quantify the effect of spatial filtering, we performed measurements with and without the iris. With the iris fully open, the harmonic spectra exhibited shot-to-shot fluctuations of $\sim 15\%$ (RMS), attributed to spatial variations in the harmonic emission pattern. With the iris closed to a diameter of $\sim 200~\mu$m (corresponding to a source region of $\sim 200~\mu$m diameter at the sample), the fluctuations were reduced to $< 5\%$ (RMS), comparable to the laser intensity noise. This demonstrates that spatial filtering significantly improves measurement stability without substantial loss of signal (the throughput with a 200~$\mu$m iris is $\sim 60\%$ of the fully open case).

\subsection{Alignment and optimization}

Alignment of the imaging assembly is performed in two steps. First, the toroidal mirrors are positioned to achieve 1:1 imaging of the sample plane onto the spectrometer entrance slit. This is verified by imaging a precision pinhole ($10~\mu$m diameter) placed at the sample position and confirming that the image size at the spectrometer entrance matches the pinhole size. Second, the iris is centered on the intermediate image by maximizing the transmitted harmonic signal while minimizing sensitivity to lateral translations of the sample.

Once aligned, the imaging assembly remains stable over extended periods (weeks to months) without requiring readjustment. This stability is facilitated by the rigid mounting of the toroidal mirrors on kinematic mounts with fine-pitch adjustment screws, and by the passive vibration isolation of the entire optical table.


==> intensity_control.tex <==
\section{Intensity control module}

Precise control of the driving-field amplitude is essential for quantitative HHG spectroscopy. In solids, the harmonic yield typically scales exponentially with field strength, making small intensity fluctuations a dominant source of systematic error in field-dependent measurements. Traditional intensity control methods---such as rotating a half-wave plate before a polarizer or adjusting pump-laser power---introduce either temporal dispersion (affecting few-cycle pulses) or beam-pointing instabilities. To circumvent these issues, we employ a dispersion-free intensity control scheme based on a pair of thin-film polarizers.

\subsection{Design and implementation}

As illustrated in Fig.~\ref{fig:intensity_control}, the module consists of two broadband thin-film polarizers (TFPs) oriented at Brewster's angle ($\sim 56^\circ$ for fused silica substrates). The first TFP (TFP1) transmits p-polarized light and reflects s-polarized light. By rotating TFP1 about the beam axis, the input polarization is decomposed into variable p- and s-components. The transmitted p-component propagates to the HHG chamber, while the reflected s-component is directed to a beam dump. The second TFP (TFP2), positioned downstream and aligned parallel to TFP1, further purifies the polarization state by rejecting residual s-polarized light, ensuring that only p-polarized radiation reaches the sample.

This configuration provides continuous intensity modulation over more than two orders of magnitude without introducing measurable temporal dispersion. Because both TFPs are thin ($\sim 1$~mm substrate thickness) and operate at Brewster's angle, group-delay dispersion and higher-order phase distortions remain negligible even for sub-5-fs pulses. Importantly, the transmitted beam direction and pointing stability are preserved across the full intensity range, as verified by monitoring the focal spot position with a high-resolution camera (see Sec.~\ref{sec:imaging}).

\begin{figure}[htbp]
\centering
\includegraphics[width=0.85\textwidth]{media/media/image2.png}
\caption{Intensity control module. Two thin-film polarizers (TFP1 and TFP2) at Brewster's angle enable dispersion-free intensity modulation. Rotation of TFP1 varies the transmitted p-polarized component, while TFP2 purifies the polarization state. The configuration preserves beam pointing and introduces negligible temporal dispersion for few-cycle pulses.}
\label{fig:intensity_control}
\end{figure}

\subsection{Performance characterization}

To quantify the dispersion introduced by the TFP pair, we performed interferometric autocorrelation measurements of few-cycle pulses ($\sim 5$~fs, 750~nm center wavelength) before and after transmission through the module. No measurable pulse broadening or spectral modification was observed across the full intensity range, confirming that the module preserves the temporal structure of ultrashort pulses. Beam-pointing stability was characterized by imaging the focal spot onto a CMOS camera while scanning the TFP1 rotation angle. The measured focal-spot centroid displacement remained below 0.5~$\mu$m over the full intensity range, well within the depth of focus and lateral extent of typical solid samples ($\sim 10$--$100~\mu$m).

The intensity modulation range depends on the extinction ratio of the TFPs and the initial polarization purity. With commercially available TFPs (extinction ratio $> 1000:1$), we routinely achieve intensity control spanning a factor of $\sim 200$ (corresponding to a field-strength range of $\sim 14$). This dynamic range is sufficient for most HHG applications, where field strengths are scanned from below threshold ($\sim 0.5$~V/\AA) to near-damage levels ($\sim 2$--$3$~V/\AA).


==> introduction.tex <==
\section{Introduction}

High-harmonic generation (HHG) in solids has evolved into a powerful spectroscopic method for probing the electronic structure across a broad range of materials. Since the first observation of HHG in bulk semiconductors under intense mid-infrared fields\cite{Ghimire2011}, the technique has been extended to dielectrics\cite{Schubert2014,Luu2015}, amorphous media\cite{Han2016}, two-dimensional semiconductors\cite{Liu2017}, gapless materials such as graphene\cite{Yoshikawa2017}, and strongly correlated and topological systems where HHG provides access to many-body dynamics, phase transitions, and surface-state responses\cite{Silva2019,Schmid2021,Uzan2020,Chacon2020}. Across these systems, the emission characteristics---cutoff energies, harmonic yields, and angular anisotropies---encode information on band structure, multiband coupling, Berry curvature, and valence-electron potentials\cite{Vampa2015,Luu2018,Lanin2017,You2017,Garg2016}. These advances establish HHG as an emerging metrological tool for quantitative solid-state spectroscopy extending from the infrared to the EUV.

Such quantitative studies, however, impose stringent requirements for adequate instrumentation. HHG yields from thin crystalline samples are highly sensitive to sample inhomogeneities and beam-pointing drifts, making field-strength scans and angular scans particularly vulnerable to systematic errors. Accurate extraction of electronic-structure information calls for (i) stable, dispersion-free control of the driving electric-field amplitude especially for few-cycle pulses, (ii) precise and reproducible crystal rotation about a well-defined axis, and (iii) simultaneous detection of harmonics across extended spectral ranges spanning from the visible to the EUV. Moreover, accurate determination of the driving-field amplitude---necessary for quantitative reconstruction of material properties---requires dedicated calibration methods\cite{Goulielmakis2008}.

In this work, we present an integrated apparatus engineered to meet these requirements for precision HHG spectroscopy in solids. The apparatus is particularly optimized for few-cycle driving fields in the near-infrared and visible parts of the spectrum. The system combines a dispersion-neutral intensity-control module, a vacuum HHG platform equipped with a custom multi-axis goniometer for sub-micrometer positioning and sub-degree rotational accuracy, an imaging and spatial filtering assembly that ensures stable focal spot interrogation during field and angle scans, and a dual-spectrometer system enabling simultaneous UV/VUV and EUV radiation detection. Absolute calibration of the driving electric field is performed via gas-phase attosecond streaking\cite{Goulielmakis2008}. Together, these capabilities constitute a versatile platform for accurate field-strength- and orientation-dependent HHG measurements, supporting a wide range of measurements in high harmonic spectroscopy of solids.


==> overview.tex <==
\section{Overview of the experimental apparatus}

The experimental apparatus (Fig.~\ref{fig:overview}) consists of four main modules: (a) the intensity control module---for precise tuning of the driving pulse intensity; (b) the high harmonic generation module---which facilitates the positioning and rotation of the crystalline specimen to be investigated at the laser beam focus; (c) the imaging and spatial filtering assembly---which enables imaging of the high harmonic source onto the entrance plane of the spectrometers, enabling also a spatial selection of harmonics emanating from specific regions of the high-harmonic beam; and (d) the detection system, where two spectrometers allow simultaneous detection of the generated harmonics in the UV/VUV and EUV ranges. Except module (a), which operates in ambient air, modules (b), (c) and (d) are housed within three interconnected chambers (Fig.~\ref{fig:overview}) maintained at a vacuum level of $10^{-6}$~mbar, allowing an absorption-free propagation of VUV and EUV harmonics from the source to the detectors. The integration of these modules establishes a platform for quantitative HHG spectroscopy, enabling high-precision field-strength and orientation-dependent measurements in bulk solids. In the following sections, we describe each module in detail.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\textwidth]{media/media/image1.png}
\caption{Schematic overview of the experimental apparatus for high harmonic spectroscopy in bulk solids. The system comprises four main modules: (a) intensity control module, (b) high harmonic generation module, (c) imaging and spatial filtering assembly, and (d) dual-spectrometer detection system. Modules (b), (c), and (d) are housed in vacuum chambers maintained at $10^{-6}$~mbar.}
\label{fig:overview}
\end{figure}

